On the freeness of the cyclotomic BMW algebras: admissibility and an isomorphism with the cyclotomic Kauffman tangle algebras

The cyclotomic Birman-Murakami-Wenzl (BMW) algebras B_n^k, introduced by R. H\"aring-Oldenburg, are a generalisation of the BMW algebras associated with the cyclotomic Hecke algebras of type G(k,1,n) (aka Ariki-Koike algebras) and type B knot theory. In this paper, we prove the algebra is free and of rank k^n (2n-1)!! over ground rings with parameters satisfying so-called "admissibility conditions". These conditions are necessary in order for these results to hold and originally arise from the representation theory of B_2^k, which is analysed by the authors in a previous paper. Furthermore, we obtain a geometric realisation of B_n^k as a cyclotomic version of the Kauffman tangle algebra, in terms of affine n-tangles in the solid torus, and produce explicit bases that may be described both algebraically and diagrammatically. The admissibility conditions are the most general offered in the literature for which these results hold; they are necessary and sufficient for all results for general n.

==> pspictures/addstring.tex <==
\mag1200
\input pstricks
\psset{unit=0.6cm}
\nopagenumbers
\vglue 5 cm
\rput(-1,0){$\iota$}
\rput(-0.5,0){:}
\psline[linestyle=dotted](0.5,1)(6.5,1)(6.5,-1)(0.5,-1)(0.5,1)
\psline[linewidth=3pt](1,1.5)(1,1)
\psline[linewidth=3pt](1,-1.5)(1,-1)
\psline(2,1.5)(2,1)
\psline(2,-1.5)(2,-1)
\psline(3,1.5)(3,1)
\psline(3,-1.5)(3,-1)
\psline(5,1.5)(5,1)
\psline(5,-1.5)(5,-1)
\psline(6,1.5)(6,1)
\psline(6,-1.5)(6,-1)
\rput(4,1.5){$\cdots$}
\rput(4,-1.5){$\cdots$}
\rput(8.5,0){$\longmapsto$}
\psline[linestyle=dotted](10.5,1)(16.5,1)(16.5,-1)(10.5,-1)(10.5,1)
\psline[linewidth=3pt](11,1.5)(11,1)
\psline[linewidth=3pt](11,-1.5)(11,-1)
\psline(12,1.5)(12,1)
\psline(12,-1.5)(12,-1)
\psline(13,1.5)(13,1)
\psline(13,-1.5)(13,-1)
\psline(15,1.5)(15,1)
\psline(15,-1.5)(15,-1)
\psline(16,1.5)(16,1)
\psline(16,-1.5)(16,-1)
\psline(17,1.5)(17,-1.5)
\rput(14,1.5){$\cdots$}
\rput(14,-1.5){$\cdots$}
\rput[b](2,1.7){$\scriptstyle 1$}
\rput[b](3,1.7){$\scriptstyle 2$}
\rput[b](5,1.7){$\scriptstyle n-2$}
\rput[b](6,1.7){$\scriptstyle n-1$}
\rput[b](12,1.7){$\scriptstyle 1$}
\rput[b](13,1.7){$\scriptstyle 2$}
\rput[b](15,1.7){$\scriptstyle n-2$}
\rput[b](16,1.7){$\scriptstyle n-1$}
\rput[b](17,1.7){$\scriptstyle n$}

\bye 

==> pspictures/affine_gen.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

\pscurve(2,1)(1.8,0.7)(1,0.3)(0.5,0)(1,-0.3)(1.8,-0.7)(2,-1)
\psline[linewidth=3 pt](1,1)(1,0.5)
\psline[linewidth=9 pt, linecolor=white](1,0.1)(1,-1)
\psline[linewidth=3 pt](1,0.1)(1,-1)

\bye 

==> pspictures/alpha1_tangle.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{xunit= .75 cm,yunit= 1 cm}
\vglue 5 cm

%\psline[linewidth=3 pt](0,0)(0,2)
\psline(1,0)(1,2)
\psline(2,0)(2,2)
  \pscurve(3,2)(3.6,1.7)(5.4,1.5)(6,2)
\psbezier[border=2pt](3,0)(3.01,0.7)(3.5,0.9)(4,2)
 \psbezier[border=2pt](4,0)(4.01,0.7)(4.5,0.9)(5,2)
 \psbezier(5,0)(5.5,0.8)(6,1.1)(7,2)
 \psbezier(6,0)(6.5,0.8)(7,1.3)(8,2)
\pscurve(7,0)(7.5,0.3)(8,0) 
\rput[t](1,2.5){$1$}
\rput[tr](3.1,2.5){$i$}
\rput[tr](6.6,2.5){$j+1$}
\rput[br](7.05,-0.47){$l$}
\rput[br](8.5,-0.5){$l+1$}
\rput[t](10,2.5){$n$}
\psline(9,0)(9,2)
\psline(10,0)(10,2)
\bye 

==> pspictures/brauer.tex <==
\mag1200
\input pstricks
\nopagenumbers
\vglue 5 cm

\qdisk(0,1){2pt}
\qdisk(1,1){2pt}
\qdisk(2,1){2pt}
\qdisk(3,1){2pt}
\qdisk(4,1){2pt}
\qdisk(0,-1){2pt}
\qdisk(1,-1){2pt}
\qdisk(2,-1){2pt}
\qdisk(3,-1){2pt}
\qdisk(4,-1){2pt}
\psbezier{->}(0,1)(0.1,0.4)(0.9,0.3)(1,0.3)
\psbezier(2,1)(1.9,0.4)(1.1,0.3)(1,0.3)
\psbezier(0,-1)(0.1,-0.4)(1.9,-0.3)(2,-0.3)
\psbezier{->}(4,-1)(3.9,-0.4)(2.1,-0.3)(2,-0.3)
\psbezier{->}(2,-1)(1.9,-0.6)(1.6,-0.6)(1.5,-0.6)
\psbezier(1,-1)(1.1,-0.6)(1.4,-0.6)(1.5,-0.6)
\psline{->}(1,1)(2,0)
\psline(2,0)(3,-1)
\psbezier{->}(4,1)(3.9,0.6)(3.6,0.6)(3.5,0.6)
\psbezier(3,1)(3.1,0.6)(3.4,0.6)(3.5,0.6)
\rput[bl](2.08,0){$\overline 2$}
\rput[bl](3,-0.3){$\overline 5$}
\rput[tl](3.95,0.8){$\overline 1$}
\rput[tr](0.05,0.8){$\overline 3$}
\rput[bl](2,-0.85){$\overline 0$}
\rput[b](0,1.2){1}
\rput[b](1,1.2){2}
\rput[b](2,1.2){3}
\rput[b](3,1.2){4}
\rput[b](4,1.2){5}
\rput[t](0,-1.2){$1'$}
\rput[t](1,-1.2){$2'$}
\rput[t](2,-1.2){$3'$}
\rput[t](3,-1.2){$4'$}
\rput[t](4,-1.2){$5'$}

\bye 

==> pspictures/closestring.tex <==
\mag1200
\input pstricks
\psset{unit=0.6cm}
\nopagenumbers
\vglue 5 cm
\rput(-1,0){${\rm cl}_n$}
\rput(-0.4,0){:}
\psline[linestyle=dotted](0.5,1)(6.5,1)(6.5,-1)(0.5,-1)(0.5,1)
\psline[linewidth=3pt](1,1.5)(1,1)
\psline[linewidth=3pt](1,-1.5)(1,-1)
\psline(2,1.5)(2,1)
\psline(2,-1.5)(2,-1)
\psline(3,1.5)(3,1)
\psline(3,-1.5)(3,-1)
\psline(5,1.5)(5,1)
\psline(5,-1.5)(5,-1)
\psline(6,1.5)(6,1)
\psline(6,-1.5)(6,-1)
\rput(4,1.5){$\cdots$}
\rput(4,-1.5){$\cdots$}
\rput(8.5,0){$\longmapsto$}
\psline[linestyle=dotted](10.5,1)(16.5,1)(16.5,-1)(10.5,-1)(10.5,1)
\psline[linewidth=3pt](11,1.5)(11,1)
\psline[linewidth=3pt](11,-1.5)(11,-1)
\psline(12,1.5)(12,1)
\psline(12,-1.5)(12,-1)
\psline(13,1.5)(13,1)
\psline(13,-1.5)(13,-1)
\psline(15,1.5)(15,1)
\psline(15,-1.5)(15,-1)
\psbezier(16,-1)(16,-3)(17,-2)(17,0)
\psbezier(16,1)(16,3)(17,2)(17,0)
\rput(14,1.5){$\cdots$}
\rput(14,-1.5){$\cdots$}
\rput(2,1.7){$\scriptstyle 1$}
\rput(3,1.7){$\scriptstyle 2$}
\rput(5,1.7){$\scriptstyle n-1$}
\rput(6,1.7){$\scriptstyle n$}
\rput(12,1.7){$\scriptstyle 1$}
\rput(13,1.7){$\scriptstyle 2$}
\rput(15,1.7){$\scriptstyle n-1$}

\bye 

==> pspictures/closure.tex <==
\mag1200
\input pstricks
\input amssym

\psset{unit=0.6cm}
\nopagenumbers
\vglue 5 cm
\rput(-2.2,0){${\rm cl}_1 \circ \ldots \circ {\rm cl}_n$}
\rput(-0.5,0){:}
\psline[linestyle=dotted](0.5,1)(6.5,1)(6.5,-1)(0.5,-1)(0.5,1)
\psline[linewidth=3pt](1,1.5)(1,1)
\psline[linewidth=3pt](1,-1.5)(1,-1)
\psline(2,1.5)(2,1)
\psline(2,-1.5)(2,-1)
\psline(3,1.5)(3,1)
\psline(3,-1.5)(3,-1)
\psline(5,1.5)(5,1)
\psline(5,-1.5)(5,-1)
\psline(6,1.5)(6,1)
\psline(6,-1.5)(6,-1)
\rput(4,1.5){$\cdots$}
\rput(4,-1.5){$\cdots$}
\rput(7.5,0){$\longmapsto$}
\psline[linestyle=dotted](8.5,1)(14.5,1)(14.5,-1)(8.5,-1)(8.5,1)
\psline[linewidth=3pt](9,1.5)(9,1)
\psline[linewidth=3pt](9,-1.5)(9,-1)
\psbezier(10,-1)(10,-6)(17,-5)(17,0)
\psbezier(10,1)(10,6)(17,5)(17,0)
\psbezier(11,-1)(11,-5.5)(16.5,-4.5)(16.5,0)
\psbezier(11,1)(11,5.5)(16.5,4.5)(16.5,0)
\psbezier(13,-1)(13,-4.5)(15.5,-3)(15.5,0)
\psbezier(13,1)(13,4.5)(15.5,3)(15.5,0)
\psbezier(14,-1)(14,-3)(15,-2)(15,0)
\psbezier(14,1)(14,3)(15,2)(15,0)
\rput(12,1.5){$\cdots$}
\rput(12,-1.5){$\cdots$}
\rput(16,0){$\cdots$}

\bye 

==> pspictures/cycloskein.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.48cm}
\vglue 5 cm
$\displaystyle
\sum_{r=0}^kq_r\hskip7pt{\cal Y}^r$
\pscircle[linestyle=dotted](-0.85,0.25){1}
${}=0$.

\bye 

==> pspictures/ebrauer.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

$e_i\quad\longmapsto{}$
%\nccurve[ArrowInside=->,ArrowInsidePos=0.5](0.8,1)(0.8,-1)
\psline{->}(0.8,1)(0.8,0)
\psline(0.8,0)(0.8,-1)
\rput(1.9,0){\dots}
\psline{->}(3,1)(3,0)
\psline(3,0)(3,-1)
\psbezier{->}(4,1)(4.25,0.7)(4.3,0.7)(4.6,0.7)
\psbezier(5,1)(4.75,0.7)(4.7,0.7)(4.6,0.7)
\psbezier{->}(4,-1)(4.25,-0.7)(4.3,-0.7)(4.6,-0.7)
\psbezier(5,-1)(4.75,-0.7)(4.7,-0.7)(4.6,-0.7)
\psline{->}(6,1)(6,0)
\psline(6,0)(6,-1)
\rput(7.1,0){\dots}
\psline{->}(8.2,1)(8.2,0)
\psline(8.2,0)(8.2,-1)
\rput(0.8,1.4){$\scriptstyle 1$}
\rput(3,1.4){$\scriptstyle i-1$}
\rput(4,1.4){$\scriptstyle i$}
\rput(5,1.4){$\scriptstyle i+1$}
\rput(6,1.4){$\scriptstyle i+2$}
\rput(8.2,1.4){$\scriptstyle n$}

\bye 

==> pspictures/emapsto.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

$e_i\longmapsto{}$
\psline[linewidth=3 pt](0,1)(0,-1)
\psline(0.8,1)(0.8,-1)
\rput(1.9,0){\dots}
\psline(3,1)(3,-1)
\pscurve(4,1)(4.5,0.5)(5,1)
\pscurve(4,-1)(4.5,-0.5)(5,-1)
\psline(6,1)(6,-1)
\rput(7.1,0){\dots}
\psline(8.2,1)(8.2,-1)
\rput(0.8,1.4){$\scriptstyle 1$}
\rput(3,1.4){$\scriptstyle i-1$}
\rput(4,1.4){$\scriptstyle i$}
\rput(5,1.4){$\scriptstyle i+1$}
\rput(6,1.4){$\scriptstyle i+2$}
\rput(8.2,1.4){$\scriptstyle n$}

\bye 

==> pspictures/kauff.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.3cm}
\vglue 5 cm

\psline(0,1)(0.8,0.2)
\psline(1.2,-0.2)(2,-1)
\psline(2,1)(0,-1)
\psline(4,1)(6,-1)
\psline(6,1)(5.2,0.2)
\psline(4.8,-0.2)(4,-1)
\rput(3,0){$-$}
\rput[l](7,0){$=\hskip4 pt\delta\Bigl[$}
\pscurve(11,1)(11.7,0)(11,-1)
\pscurve(13,1)(12.3,0)(13,-1)
\pscurve(15,1)(16,0.3)(17,1)
\pscurve(15,-1)(16,-0.3)(17,-1)
\rput(14,0){$-$}
\rput[l](18.1,0){$\Bigr]$}


\bye 

==> pspictures/reid1.tex <==
\mag1200
\input pstricks
\mag1200
\nopagenumbers
\psset{unit=0.48cm}
\vglue 5 cm

\pscurve(0,1)(0.6,-0.3)(0.9,0)(0.6,0.3)(0.4,0.2)
\pscurve(0.2,-0.2)(0.1,-0.5)(0,-1)
\rput[l](1.7,0){$\leftrightarrow$}
\psline(3.6,1)(3.6,-1)
\rput(5,0){$\leftrightarrow$}
\pscurve(6.2,-1)(6.8,0.3)(7.1,0)(6.8,-0.3)(6.6,-0.2)
\pscurve(6.4,0.2)(6.3,0.5)(6.2,1)

\bye 

==> pspictures/reid3.tex <==
\mag1200
\input pstricks
\mag1200
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

\psbezier(2,1)(2,0)(0,1)(0,-1)
\psbezier(0,1)(0,0.7)(0,0.2)(0.15,0.05)
\psbezier(0.45,-0.05)(1,-0.1)(2,0)(2,-1)
\psline[linecolor=white, linewidth=4pt](1,1)(1,-1)
\psline(1,1)(1,-1)
\rput(3,0){$\leftrightarrow$}
\psbezier(4,-1)(4,0)(6,-1)(6,1)
\psbezier(6,-1)(6,-0.7)(6,-0.2)(5.85,-0.05)
\psbezier(5.55,0.05)(5,0.1)(4,0)(4,1)
\psline[linecolor=white, linewidth=4pt](5,1)(5,-1)
\psline(5,1)(5,-1)

\bye


==> pspictures/untwist.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.4cm}
\vglue 5 cm

\pscurve(0,1)(0.6,-0.3)(0.9,0)(0.6,0.3)(0.4,0.2)
\pscurve(0.2,-0.2)(0.1,-0.5)(0,-1)
\rput[l](1.5,0){$=\hskip2 pt\lambda$}
\psline(3.5,1)(3.5,-1)
\rput(7,0){and}
\pscurve(10,-1)(10.6,0.3)(10.9,0)(10.6,-0.3)(10.4,-0.2)
\pscurve(10.2,0.2)(10.1,0.5)(10,1)
\rput[l](11.5,0){$=\hskip2 pt\lambda^{-1}$}
\psline(14.4,1)(14.4,-1)

\bye

==> pspictures/xbrauer.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

$X_i\quad\longmapsto{}$
\rput(0.1,0.1){$\lambda$}
\psline{->}(0.8,1)(0.8,0)
\psline(0.8,0)(0.8,-1)
\rput(1.9,0){\dots}
\psline{->}(3,1)(3,0)
\psline(3,0)(3,-1)
\psline{->}(4,1)(4.4,0.2)
\psline(4.4,0.2)(5,-1)
\psline{->}(5,1)(4.6,0.2)
\psline(4.6,0.2)(4,-1)
\psline{->}(6,1)(6,0)
\psline(6,0)(6,-1)
\rput(7.1,0){\dots}
\psline{->}(8.2,1)(8.2,0)
\psline(8.2,0)(8.2,-1)
\rput(0.4,0.1){$\left[\vrule height 0.6cm depth 1cm width 0pt\right.$}
\rput(8.7,0.1){$\left.\vrule height 0.6cm depth 1cm width 0pt\right]$}
\rput(0.8,1.4){$\scriptstyle 1$}
\rput(3,1.4){$\scriptstyle i-1$}
\rput(4,1.4){$\scriptstyle i$}
\rput(5,1.4){$\scriptstyle i+1$}
\rput(6,1.4){$\scriptstyle i+2$}
\rput(8.2,1.4){$\scriptstyle n$}

\bye 

==> pspictures/xmapsto.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

$X_i\longmapsto{}$
\psline[linewidth=3 pt](0,1)(0,-1)
\psline(0.8,1)(0.8,-1)
\rput(1.9,0){\dots}
\psline(3,1)(3,-1)
\psline(4,1)(4.4,0.2)
\psline(4.6,-0.2)(5,-1)
\psline(5,1)(4,-1)
\psline(6,1)(6,-1)
\rput(7.1,0){\dots}
\psline(8.2,1)(8.2,-1)
\rput(0.8,1.4){$\scriptstyle 1$}
\rput(3,1.4){$\scriptstyle i-1$}
\rput(4,1.4){$\scriptstyle i$}
\rput(5,1.4){$\scriptstyle i+1$}
\rput(6,1.4){$\scriptstyle i+2$}
\rput(8.2,1.4){$\scriptstyle n$}

\bye 

==> pspictures/ybrauer.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

$\quad Y\quad \longmapsto$
\rput[tl](0.5,0.5){$\overline 1$}
\psline{->}(1,1)(1,0)
\psline(1,0)(1,-1)
\psline{->}(2,1)(2,0)
\psline(2,0)(2,-1)
\rput(3,0){\dots}
\psline{->}(4,1)(4,0)
\psline(4,0)(4,-1)
\rput[b](1,1.2){$\scriptstyle 1$}
\rput[b](2,1.2){$\scriptstyle 2$}
\rput[b](4,1.2){$\scriptstyle n$}

\bye 

==> pspictures/ymapsto.tex <==
\mag1200
\input pstricks
\nopagenumbers
\psset{unit=0.72cm}
\vglue 5 cm

$Y\mapsto$
\pscurve(2,1)(1.8,0.7)(1,0.3)(0.5,0)(1,-0.3)(1.8,-0.7)(2,-1)
\psline[linewidth=3 pt](1,1)(1,0.5)
\psline[linewidth=9 pt, linecolor=white](1,0.1)(1,-1)
\psline[linewidth=3 pt](1,0.1)(1,-1)
\psline(3,1)(3,-1)
\rput(4,0){\dots}
\psline(5,1)(5,-1)
\rput[b](2,1.2){$\scriptstyle 1$}
\rput[b](3,1.2){$\scriptstyle 2$}
\rput[b](5,1.2){$\scriptstyle n$}

\bye 
